HopsFS: Scaling Hierarchical File System Metadata Using NewSQL Databases

Recent improvements in both the performance and scalability of shared-nothing, transactional, in-memory NewSQL databases have reopened the research question of whether distributed metadata for hierarchical file systems can be managed using commodity databases. In this paper, we introduce HopsFS, a next generation distribution of the Hadoop Distributed File System (HDFS) that replaces HDFS' single node in-memory metadata service, with a distributed metadata service built on a NewSQL database. By removing the metadata bottleneck, HopsFS enables an order of magnitude larger and higher throughput clusters compared to HDFS. Metadata capacity has been increased to at least 37 times HDFS' capacity, and in experiments based on a workload trace from Spotify, we show that HopsFS supports 16 to 37 times the throughput of Apache HDFS. HopsFS also has lower latency for many concurrent clients, and no downtime during failover. Finally, as metadata is now stored in a commodity database, it can be safely extended and easily exported to external systems for online analysis and free-text search.

==> fsopstodbops.tex <==
\subsection{Effect of DB Optimization Techniques}
%We have employed different database techniques to increase throughput as discussed in  %\cref{sec:paritioning-metadata}. 
In this experiment, we focus on three optimizations; (1) distribution aware transactions (DAT),~\cref{sec:paritioning-metadata}, (2) application defined partitioning (ADP),~\cref{sec:paritioning-metadata}, and (3) the inode hint cache at the namenodes, \cref{sec:namenodes-cache}. We ran file creation and file read experiments on a 12 namenode HopsFS cluster while varying the file depth, as shown in Figures~\ref{fig:hops-optimizations-file-reading}~and~\ref{fig:hops-optimizations-file-writing}.

\input{ops-table.tex}

File system operations in HopsFS are implemented as one or more transactions, where each transaction performs multiple round trips to the database to read and update the metadata. In Table \ref{table:fsopstodbops}, we show the number of round trips needed for each operation in the case of (1) no inode hint cache and (2) inode hint cache hits. For example, if we create an empty file \textit{/d1/d2/.../d9/f} at depth $N=10$, then in the case of no caching, we substitute in the equation from Table \ref{table:fsopstodbops} and derive the cost of the operation as $17PK_{rc} + 5PK_{w} + 2PPIS +2B_{1}$, that is $26$ round trips to the database. In contrast, in the case of cache hits for all inodes hints, we will have $11$ round trips to the database, irrespective of the depth of the file in the namespace hierarchy. Cache hits save $15$ round trips, giving an expected $58\%$  performance improvement for the file create operation. We validated our analysis of the file system operations by running experiments for both cases, that is, with the cache enabled \textit{(HopsFS-DAT+ADP+Cache)} and with the cache disabled \textit{(HopsFS-DAT+ADP)}, as shown in Figure~\ref{fig:hops-optimizations-file-writing}. Our experiments show that at depth $N=10$ the inode cache improves HopsFS' throughput for file creation by $\approx 58\%$. Similarly, in the case of file read, the cache improves HopsFS by $\approx 68\%$, see Figure \ref{fig:hops-optimizations-file-reading}.


\begin{figure}[t]
\includegraphics[width=0.48\textwidth]{imgs/compiled-results/4NDB/incremental-optimizations/get_block_location_optimizations.pdf}
 \caption{Effect of different optimizations on file read operation with respect to depth of the file in the namespace hierarchy}
 \label{fig:hops-optimizations-file-reading}
 \end{figure}
 \begin{figure}[t]
 \includegraphics[width=0.48\textwidth]{imgs/compiled-results/4NDB/incremental-optimizations/create_file_optimizations.pdf}
 \caption{Effect of different optimizations on file create operation with respect to depth of the file in the namespace hierarchy.}
 \label{fig:hops-optimizations-file-writing}
 \end{figure}
  


==> ops-table.tex <==
\begin{table*}[t]
\scriptsize
\begin{tabular}{| p{0.055\textwidth}   p{0.49\textwidth}   p{0.4\textwidth} |}
\hline
\hline
\cellcolor{tableHeaderColor}\textbf{ FS Ops} & \cellcolor{tableHeaderColor}\textbf{ Without Inode Hint Cache at the NameNodes} & \cellcolor{tableHeaderColor}\textbf{ Inode Hint Cache Hits} \\
\hline
\hline
\rowcolor{lightRowColor}mkdirs($d_{N}$) & $(N-2)PK_{rc}+2PK_{w} +B_{1}$ & $2PK_{w} + (2B)_{N-1}$ \\
%\hline
\rowcolor{darkRowColor}addBlk($f_{N}$) & $(N-1)PK_{rc} + PK_{w} + PK_{r} + B_{1} + (f_{s}==0 \ ? \ 2PPIS \ :\ 6PPIS)$ & $PK_{w} + PK_{r} + (2B)_{N}+ (f_{s}==0 \ ? \ 2PPIS \ :\ 6PPIS)$ \\

\rowcolor{lightRowColor}create($f_{N}$) & $(2N-3)PK_{rc} + 5PK_{w} + 2B_{1} + (f_{s}==0 \ ? \ 2PPIS \ :\ 8PPIS) + \sum\limits_{b=b_{0}}^{b_{x}} \text{addBlk(}f_{N}\text{)} $ & $5PK_{w} + (4B)_{2N-1} + (f_{s}==0 \ ? \ 2PPIS \ :\ 8PPIS) + \sum\limits_{b=b_{0}}^{b_{x}} \text{addBlk(}f_{N}\text{)}$ \\
%\hline 
%append($f_{N}$) & $(3N-4)PK_{rc} +5PK_{w} + PK_{r} + 16PPIS + 3B_{1} + \sum\limits_{b=b_{0}}^{b_{x}} \text{addBlock(}b, f_{N}\text{)}$ & $5PK_{w}+ +PK_{r} + 16PPIS +(6B)_{3N-1} + \sum\limits_{b=b_{0}}^{b_{x}} \text{addBlock(}b, f_{N}\text{)}$ \\
%\hline
\rowcolor{darkRowColor}read($f_{N}$)  & $(N-1)PK_{rc} + PK_{r} + B_{1} + (f_{s} == 0 \ ? \ PPIS \ :\ 5PPIS)$ & $PK_{r} + (2B)_{N} + (f_{s}==0 \ ? \ PPIS \ :\ 5PPIS)$ \\
%\hline
\rowcolor{lightRowColor}ls($i_{N}$) & $(N-1)PK_{rc} + PK_{r} + (i \text{ is a dir}\ ? \ PPIS \ :\ 0) $ & $PK_{r} + B_{N-1} + (i \text{ is a dir}\ ? \ PPIS \ :\ 0) $ \\ 
%\hline
\rowcolor{darkRowColor}chmod($i_{N}$) & $(2N-2)PK_{rc} +2PK_{w} + 2B_{1} + (i \text{ is a dir}\ ? \ IS \ :\ PPIS) $ & $2PK_{w} + (4B)_{2N} + (i \text{ is a dir}\ ? \ IS \ :\ PPIS)$\\
%\hline
%setRepl($f_{N}$) & $(N-2)PK_{rc} + 2PK_{w} + 7PPIS + B_{1}$ & $2PK_{w} + 7PPIS + (2B)_{N-1}$ \\
%\hline
\rowcolor{lightRowColor}info($i_{N}$) & $(N-1)PK_{rc} + PK_{r} + B_{1}$ & $PK_{r} + (2B)_{N}$ \\
%\hline
%chown($i_{N}$) & $(2N-2)PK_{rc} + 2PK_{w} + 2B_{1} + (i \text{ is a dir}\ ? \ IS \ :\ PPIS)$ & $2PK_{w} + (4B)_{2N} + (i \text{ is a dir}\ ? \ IS \ :\ PPIS)$\\
%\hline
\rowcolor{darkRowColor}del($f_{N}$) & $(2N-2)PK_{rc} + 2PK_{w} + 2B_{1} + (f_{s}==0 \ ? \ 2PPIS \ :\ 7PPIS)$ & $2PK_{w} + (4B)_{2N} + (f_{s}==0 \ ? \ 2PPIS \ :\ 7PPIS)$\\
%\hline
\rowcolor{lightRowColor}delTree($i_N$) & $(N -2) PK_{rc} + 2PK_{w} + B_{1} + (i_{s}==0\ |\ i \text{ is a dir}\ ? \ PPIS \ :\ 7PPIS) $ & $2PK_{w} + (2B)_{N-1} + (i_{s}==0 \ |\ i \text{ is a dir}\ ? \ PPIS \ :\ 7PPIS)$ \\

\rowcolor{darkRowColor}del($d_{N}$) & $(3N-1)PK_{rc} + 2PK_{w} + 3B_{1} + IS + \sum\limits_{i=f_{1}}^{f_{x}} \text{delTree(}i_{N}\text{)}$ & $2PK_{w} + (3B)_{3N+1} + IS + \sum\limits_{i=f_{1}}^{f_{x}} \text{delTree(}i_{N}\text{)}$ \\
%\hline
\rowcolor{lightRowColor}mv($f_{N}$,$f_{M}$) & $(2M+2N-S-4)PK_{rc} + (3B)_{4} +(f_{s}==0 \ ? \ 2PPIS \ :\ 9PPIS)+ (S==M-1\ \&\ M==N \ ? \ 3PK_{w} \ :\ 4PK_{w})$ & $ (7B)_{2M+2N-S} +(f_{s}==0 \ ? \ 2PPIS \ :\ 9PPIS) + (S==M-1\ \&\ M==N \ ? \ 3PK_{w} \ :\ 4PK_{w})$\\
%\hline
\rowcolor{darkRowColor}mv($d_{N}$,$d_{M}$) &$(2M+3N-S-5)PK_{rc} + 2IS + (4B)_{5} +  (S==M-1\ \&\ M==N \ ? \ 4PK_{w} \ :\ 5PK_{w})$& $ 2IS + (8B)_{2M+3N-S} + (S==M-1\ \&\ M==N \ ? \ 4PK_{w} \ :\ 5PK_{w})$\\
\hline
\hline
\end{tabular}
\\
%\begin{tabular}{ l l l l }
\begin{tabular}{ p{0.05\textwidth}   p{0.5\textwidth}  p{0.02\textwidth}  p{0.38\textwidth} }

$f_{N}$,$d_{N}$,$i_{N} :$ & $f$=file, $d$=dir, $i$=file/dir path at depth $N$  &
$f_{s} :$ & size of a file $f$ \\
$PK_{w}$,$PK_{rc} :$ & a primary key read operation with a \underline{w}rite or a \underline{r}ead-\underline{c}ommitted lock (i.e., no lock) &
$PPIS :$ & a partition pruned index scan \\
$xB_{N} :$ & $x$ primary key batch operations that read in total $N$ rows from the database &
$FTS :$ & Full table scan without using indexes (hits all shards) \\
$S :$ & number of shared inodes in the paths between ($f_{N}$ and $f_{M}$) or ($d_{N}$ and $d_{M}$) &
$ IS :$ & Index scan (hits all shards) \\
\end{tabular}

\caption{The cost of file system (metadata) operations in terms of database accesses for (1) no inode hint caching and (2) cache hits. }
\label{table:fsopstodbops}
\vspace{2mm}
\hrulefill
\vspace{-4mm}
\end{table*}


==> problem.tex <==
\section{The BIG Problem}
The Hadoop platform has received tremendous attention from the research community in recent years. This is due to the fact that it is the most advanced and complete open-source ecosystem for big data analytics. However, the Hadoop Distributed File System (HDFS) \cite{shvachko2010Hdfs} has received relatively less attention from the research community. The core design of HDFS namenode has not changed since the project was first started: a single namenode is responsible for the maintenance of the entire file system metadata.

In order to reduce the software complexity of the namenode and ensure its correctness and performance, the entire file system metadata is stored in the main memory of the namenode. This makes it very simple to implement the file system operations, but this is not scalable and become a limitation for the platform. In fact, Hadoop clusters can grow very large and a single namenode will have to serve thousands of datanodes and hundreds of thousands of clients simultaneously while storing tens of gigabytes of metadata in RAM.

The problem with storing the namespace metadata in memory is two-fold. First, the namespace metadata cannot grow more than the main memory of the namenode. Secondly, when the in-memory metadata grows to tens of gigabytes the application performance degrades due to JVM stop-the-world garbage collection events. Java garbage collectors are infamous for their poor performance for large heap sizes: the garbage collection thread consumes a significant amount of CPU resources and can pause applications for seconds at a time \cite{shvachko2010HDFSlimitations}.

Moreover the namespace metadata is kept strongly consistent using \emph{readers-writer} concurrency semantics, implemented using a global namespace lock. All the write operations are serialized, even if these operations intend to mutate different files in the different sub-trees of the namespace hierarchy. A write operation blocks all other operations; and a large write operation can potentially block the namespace for a very long time. Some operators have reported that due to sudden influx of \emph{write}-operations and JVM stop-the-world garbage collection, the namenode can become unresponsive for tens of minutes \cite{spotify_gc_problem}. Due to the coarse grained NameSystem lock the namenode doesn't scale well on multi-core hardware and the CPU is often underutilized for \emph{write} intensive workloads \cite{BLOG_HDFS_CENTRAL_LOCK, JIRA_HDFS_1093}.

Storing all the namespace data on a single namenode also makes the file system highly vulnerable. The file system becomes inaccessible when the namenode fails. Hadoop solves this problem with a hot swappable Standby namenode that takes over as soon as it detects that the Active namenode has failed. Yet, the time needed to propagate the logs from the main namenode to the standby one is not negligible. From the time of detection of failure of the Active namenode, the standby node can take tens of seconds to apply all the outstanding logs entries before serving read and write operations. Moreover, having a standby namenode does not completely solve the single point of failure problem, the system can only tolerate a single namenode failure. In case of failure of the Active namenode, the standby namenode becomes a single point of failure until the cluster administrators revive the failed Active namenode. Although this problem can be resolved with even more redundant hardware (a standby for the standby), the costs involved and the fact the hardware does not contribute to the file system during normal operation, mean that operators typically go with just Active and Standby namenodes.

Another problem with the Apache implementation of the namenode is that it sometimes returns inconsistent results. Whenever the namenode receives a write request it performs following steps:
\iffalse
\begin{enumerate}
 \item acquires exclusive locks on the NameSystem,
 \item performs permission checks and updates the namespace,
 \item releases the Namespace lock,
 \item saves the changes in the EditLog, and
 \item finally, it notifies the client of the result of the operation. 
\end{enumerate}

As soon as the namenode releases the namespace lock, the changes become visible to other clients and operations in the system. This can lead to inconsistent read operations. For example, consider a scenario where a client \emph{A} creates a file \emph{F}. The namenode makes the changes in the namespace and releases the namespace lock. The new file is now visible to the other clients in the system and a client \emph{B} can read the file. If the namenode fails before it persisted the creation of \emph{F} in the Journal Nodes, the standby namenode will take over without any information about the creation of the new file \emph{F}. If the client \emph{B} tries to read the file \emph{F} again will receive an error indicating that the file does not exist. Such inconsistencies arise because of the premature release of the namespace lock before changes to the namespace have been persisted. To strengthen the namenode's consistency semantics, the namespace locks should only be released once the changes have been persisted in the EditLog. But persisting to the EditLog is slow (tens of milliseconds) and holding the namespace lock while the file system changes are persisted would massively decrease the throughput of the namenode. The designers surmised that weaker-than-Posix semantics are tolerable for users, given the increased performance it brings.

There is great need for a file system metadata management that is highly available, scales horizontally, and supports multiple concurrent write changes to the file system metadata. In this paper we present our distribution of HDFS called HopsFS. HopsFS achieves horizontal scalability of metadata management by making the namenode stateless. All the metadata is stored in a highly available, highly performant distributed database. This allows HopsFS to have multiple stateless namenodes which can process operations in parallel. The cluster administrator can increase or decrease the number of namenodes depending on the workload and SLA requirements. All the clients in the system uniformly distribute their file system operations among all the namenodes.

HopsFS supports fine-grained \emph{readers-writers} concurrency locking while strengthening the consistency semantics of HDFS. Unlike Apache HDFS, that locks the entire namespace to keep the namespace consistent, HopsFS takes locks on the individual files or dreictories affected by each file system operation. This allows us to perform multiple file system read and write operations in parallel. Fine-grained locking and ACID transactions ensure that multiple namespace changes do not violate the consistency of the file system.
\fi
